Paint and Distill: Boosting 3D Object Detection with Semantic Passing Network

3D object detection task from lidar or camera sensors is essential for autonomous driving. Pioneer attempts at multi-modality fusion complement the sparse lidar point clouds with rich semantic texture information from images at the cost of extra network designs and overhead. In this work, we propose a novel semantic passing framework, named SPNet, to boost the performance of existing lidar-based 3D detection models with the guidance of rich context painting, with no extra computation cost during inference. Our key design is to first exploit the potential instructive semantic knowledge within the ground-truth labels by training a semantic-painted teacher model and then guide the pure-lidar network to learn the semantic-painted representation via knowledge passing modules at different granularities: class-wise passing, pixel-wise passing and instance-wise passing. Experimental results show that the proposed SPNet can seamlessly cooperate with most existing 3D detection frameworks with 1~5% AP gain and even achieve new state-of-the-art 3D detection performance on the KITTI test benchmark. Code is available at: https://github.com/jb892/SPNet.

==> Section/3-method.tex <==
\section{Methodology}

\begin{figure*}[t]
 \begin{center}
  \includegraphics[width=0.9\textwidth]{Figures/acm_mm_2022_spnet_framework.pdf}
 \end{center}
 \caption{
    The overview of our \networkname framework. Firstly, for each LiDAR point cloud sample input, we apply GT-Painting method to create the semantic mask for each point and concatenate with the raw point cloud. Then, we feed raw and masked point cloud into the student and teacher model respectively. The semantic information contain inside the teacher network is passed to student network through three different granularity levels $\{\mathcal{V}_{3d}$, $\mathcal{F}_{BEV}$, $\mathcal{P}_{cls} \}$ by three passing modules: \distillmethodone, \distillmethodtwo and \distillmethodthr.
 }
 \label{spnet_framework}
\end{figure*}

In this work, to improve the performance of our baseline 3D detector, we developed two main strategies to utilize the semantic information contained inside the ground-truth bounding boxes (GT bboxes).  Firstly, we train a strong baseline detector by using the semantic foreground masks created by GT bboxes.  Secondly, we employ the strong baseline detector as teacher to guide the training of the student model with the identical network structure. To minimize the performance gap between teacher and student detector, we established \networkname framework which primarily consists of three information passing modules: \distillmethodone, \distillmethodtwo and \distillmethodthr. 

In the following section, we shall introduce the GT-Painting method in Sec. \ref{1}. Then, we describe the proposed \networkname framework architecture in details in Sec. \ref{2}. In the last Sec. \ref{3}, we further explain the training process of \networkname.




\subsection{GT-Painting}
\label{1}

% \begin{figure}[htb]
%  \begin{center}
%   \includegraphics[width=7.5cm]{Figures/painting_result_comp_chart.pdf}
%  \end{center}
%  \caption{
%   Comparison between the performance of  PointPainting\cite{vora2020pointpainting} and our GT-Painting method on Kitti validation datset with 3D
%   Object Detection scores on Car. The baseline model is PointPillars\cite{lang2019pointpillars}.
%  }
%  \label{fig2}
% \end{figure}

As we mentioned in the introduction section, the idea behind the  PointPainting\cite{vora2020pointpainting} is to give each input point a the semantic label from the 2D semantic segmentation result of the relevant RGB image. So, that the 3D detector can take advantage of the semantic information and achieve better result. However, through our observation, the performance of such painting method is largely dependent on the quality of semantic segmentation result. The painting method could bring 2\% mAP performance improvement if we use a very strong 2D semantic segmentation model like HRNet-OCR\cite{YuanCW19}. The improvement vanished if we only use the original HRNet\cite{SunXLW19}. So, we wonder what is the performance upper bound of the PointPainting method if we could provide a theoretically best semantic mask? This can be achieved by directly using the ground-truth bounding box to create the semantic mask. It is  described in following section.

For each input point cloud $\mathcal{D}_{raw} \in \mathbb{R}^{N\times C}$, $C\geq 3$, the semantic binary mask $\mathcal{M}_{sem}\in \mathbb{R}^{N\times 1}$ is generated by testing if each point is in the GT bboxes or not. The points inside the bounding boxes are marked as foreground with numerical figure 1. Otherwise, the points are marked as background with numerical value 0. Then, we channel-wisely concatenate the raw point cloud $L$ with the semantic binary mask $\mathcal{M}_{sem}$ to get input $\mathcal{D}_{sem}$. Finally, we feed it into the pointpillars model for training. Compared to baseline model, the performance of the GT-Painting method achieves about 10.47\% increase on Kitti validation benchmark. So, the performance upper bound of the painting method is found. But, how can we utilize this painting method without being bottle-necked by the 2D semantic segmentation network? We choose to introduce the distillation framework \networkname by passing rich semantic information learnt by the teacher model to the student model to improve the performance of the 3D Detector.

% The 2D semantic segmentation network becomes the bottleneck of the performance of the  PointPainting method. It also brings tremendous amount of the computational cost during inference time which makes it impractical for real-world applications. 

\subsection{\networkname Architecture}
\label{2}
% \subsubsection{Overview}




\textbf{Overview.} The proposed \networkname framework structure is shown in Fig. \ref{spnet_framework}. Theoretically, the \networkname framework can be applied to any main stream 3D detection models. In this diagram, we describe our method by using PointPillars\cite{lang2019pointpillars} as our baseline model. In addition, the student and teacher model share the same structure. Firstly, our teacher model is pre-trained on GT-Painted point clouds which contains rich semantic information at different levels. After that, we exploit our \networkname to train the student model by passing semantic information through three granularity levels. The first passing level is at the $\mathcal{V}_{3d}$ volume feature which is the output of the 3D backbone encoder that usually encodes sparse 3D features. We design a \distillmethodone module to imitate the inner-class feature distributions between student and teacher. The second passing level is at the output feature $\mathcal{F}_{bev}$ of 2D backbone encoder. We apply the \distillmethodtwo module to minimize the distance between the medium-level features. The last passing module is act on the output class prediction score map $\mathcal{P}_{cls}$ of the rpn module. It is the finest-level of supervision to student model provided by teacher branch.

\textbf{Class-wise Passing Module.} In order to effectively make the student model learn the semantic information contained inside the teacher model, we first design a \distillmethodone module to minimize the differences between the inner-class feature distribution of $\mathcal{V}^{S}_{3d}$ and $\mathcal{V}^{T}_{3d}$. The \distillmethodone module can be divided into 5 steps. It takes $\mathcal{V}^S_{3d} \in \mathbb{R}^{H\times W\times D\times C}$ and $\mathcal{V}^T_{3d} \in \mathbb{R}^{H\times W\times D\times C}$ features as input. Step 1, both features are compressed along the gravitational dimension $D$ to get the BEV shape feature $\mathcal{V}_{3d}\in \mathbb{R}^{H\times W\times D\times C} \rightarrow \tilde{\mathcal{V}}_{3d}\in \mathbb{R}^{H\times W\times K}\text{, where }K = D\times C$. At step 2, to compute the binary foreground mask $\mathcal{M}^C_{fg}\in \mathbb{R}^{H\times W}\text{ and background mask } \mathcal{M}^C_{bg}\in \mathbb{R}^{H\times W} \text{, where }C$ is number of object classes. Step 3, to find the inner-class global feature $\mathcal{F}_{global}\in \mathbb{R}^{H\times W\times K}$ for both teacher and student features of each class in Eq. \ref{eq_inner_class_global_feat}. The normalization in step 3 is done by adding up the binary mask values along $H$, $W$ dimension and divide along $K$ dimension.

\begin{equation}
\begin{aligned}
\mathcal{F}^{T,C}_{global} = \mathcal{M}^C_{bg} \cdot \tilde{\mathcal{V}}^T_{3d} + \left \| \mathcal{M}^C_{fg}\cdot \tilde{\mathcal{V}}^T_{3d}\right \|_{norm} \\
\mathcal{F}^{S,C}_{global} = \mathcal{M}^C_{bg} \cdot \tilde{\mathcal{V}}^S_{3d} + \left \|\mathcal{M}^C_{fg}\cdot \tilde{\mathcal{V}}^S_{3d}\right \|_{norm}
\end{aligned}
 \label{eq_inner_class_global_feat}
\end{equation}

Step 4, to form the cosine similarity matrix $\mathcal{A}\in \mathbb{R}^{H\times W}$ for both teacher and student features of each class in Eq. \ref{eq_cos_similar_matrix}. The $\epsilon$ value is 1e-6 to prevent zero division. 

\begin{equation}
\begin{aligned}
\mathcal{A}^{T, C} = \frac{\tilde{\mathcal{V}}^T_{3d}\cdot \mathcal{F}^{T,C}_{center}}{max\left ( \left \|  \tilde{\mathcal{V}}^T_{3d}\right \|_2\cdot \left \| \mathcal{F}^{T,C}_{center} \right \|_2, \epsilon \right )} \\
\mathcal{A}^{S, C} = \frac{\tilde{\mathcal{V}}^S_{3d}\cdot \mathcal{F}^{S,C}_{center}}{max\left ( \left \|  \tilde{\mathcal{V}}^S_{3d}\right \|_2\cdot \left \| \mathcal{F}^{S,C}_{center} \right \|_2, \epsilon\right )}
\end{aligned}
 \label{eq_cos_similar_matrix}
\end{equation}

Step 5, to calculate the \distillmethodone loss $\mathcal{L}_c$ between cosine similarity matrix of teacher and student in Eq. \ref{eq_loss_group}.

% The experimental results show that the class-wise global affinity map loss outperforms the other two losses. We shall discuss it in the experiment section \ref{}.
% three different kinds of imitation losses \{ L1\_loss, affinity map loss, group-wise passing loss \}

% \begin{equation}
% \mathcal{L}_c = \frac{1}{H\times W}\sum^{H}_{i}\sum^{W}_{j}\sum^{C}_{q}\left \| \mathcal{A}^{T, q}_{i,j} - \mathcal{A}^{S, q}_{i, j} \right \|_2
%  \label{eq_loss_group}
% \end{equation}

\begin{equation}
\mathcal{L}_c = \sum^{C}_{q}\left \| \mathcal{A}^{T, q}_{i,j} - \mathcal{A}^{S, q}_{i, j} \right \|_2
 \label{eq_loss_group}
\end{equation}

\textbf{Feature-wise Passing Module} The \distillmethodtwo module takes the BEV feature map $\mathcal{F}_{bev}$ of teacher and student model as input. By minimizing the L2 distance between two feature maps, the semantic information flow from teacher to student spatially. However, the background regions often occupy a significant amount of contribution in feature loss which is unnecessary and make the \distillmethodtwo module less effective. So, we create a foreground binary feature mask $\mathcal{M}_{fg}$ by using the GT bboxes to make the loss calculation only focused on foreground area. The loss function is show in Eq. \ref{eq_loss_feature}.

\begin{equation}
\mathcal{L}_f = \mathcal{M}_{fg} \cdot \left \| \mathcal{F}^T_{bev} - \mathcal{F}^S_{bev} \right \|_2
\label{eq_loss_feature}
\end{equation}

\textbf{Prediction-wise Passing Module.} The \distillmethodthr module helps to increase the consistency between teacher and student branches in prediction level. Many pioneer works \cite{wang2019distilling,guo2021distilling,zhou2021sgm3d} have proven that label generated from a better domain can provide additional knowledge guidance at fine-grained level of supervision instead of only using hard labels as direct supervision. The input of the \distillmethodthr module are the class prediction score map $\mathcal{P}_{cls} \in \mathbb{R}^{H\times W \times A}$ of teacher and student model. $A$ is the number of anchors at each prediction grid. Our method is described in Eq. \ref{eq_prediction_wise_loss}. First, we adopt masked Kullback-Leibler(KL) divergence loss \ref{eq_kld_loss} to compute the distance between teacher and student prediction for both foreground and background. Then, we re-weight the foreground and background loss by using empirical value $\lambda_{fg}$ and $\lambda_{bg}$ respectively. Finally, we add up two losses to get the final loss for \distillmethodthr module.

\begin{equation}
\begin{aligned}
\mathcal{L}_{p} = \lambda_{fg} \cdot KLD \left ( \mathcal{P}^{T}_{cls}, \mathcal{P}^{S}_{cls}, \mathcal{M}_{fg}\right ) + \\
\lambda_{bg} \cdot KLD\left ( \mathcal{P}^{T}_{cls}, \mathcal{P}^{S}_{cls}, \mathcal{M}_{bg}\right )
 \end{aligned}
 \label{eq_prediction_wise_loss}
\end{equation}

The masked K-L divergence loss In equation \ref{eq_kld_loss}, we describe 

\begin{equation}
KLD\left ( \mathcal{F}^t, \mathcal{F}^p, \mathcal{M}\right ) = \frac{\sum (\mathcal{M}\cdot\mathcal{F}^t \cdot (log\mathcal{F}^t - log\mathcal{F}^p))}{max\left ( \sum \mathcal{M}, \epsilon \right )}
 \label{eq_kld_loss}
\end{equation}



\textbf{Extra train and inference detail.} During training stage, the final loss function \ref{eq_loss_total} consists of two components: 1) the RPN loss produced by the student model which supervised by ground-truth bounding boxes. 2) the distill losses from three information passing modules. The weight of pre-trained teacher model is frozen and not involved in the training process. The weights of student model are initialized randomly and trained from scratch. Only student branch is activated during inference time. Thus, there is no extra computational cost for any detector model wanna apply our method to improve the performance.

\begin{equation}
\mathcal{L}_{total} = \mathcal{L}^{S}_{rpn} + \lambda_g\cdot\mathcal{L}_{c} + \lambda_f\cdot\mathcal{L}_{f} + \lambda_p\cdot\mathcal{L}_{p}
 \label{eq_loss_total}
\end{equation}


